MeerKAT view of Hickson Compact Groups: II. HI deficiency in the core and surrounding regions

Hickson compact groups (HCGs) offer an ideal environment for investigating galaxy transformation as a result of interactions. It has been established that the evolutionary sequence of HCGs is marked by an intermediate stage characterised by a substantial amount of HI in their intragroup medium (IGrM) in the form of tidal tails and bridges (Phase 2), rapidly followed by a final stage where no IGrM gas is found and where their member galaxies are highly HI-deficient (Phase 3). Despite numerous single-dish and interferometric HI studies on the HCGs, a clear HI picture of the groups within their large-scale environment still remains to be uncovered. Taking advantage of the MeerKAT's high column density sensitivity and large field-of-view, we aim to investigate the rapid transformation of HCGs from the intermediate to late phases, and establish a picture of their gas content variations in the context of their large-scale environments. We performed MeerKAT observations of six HCGs selected to represent the intermediate and late phases of the proposed evolutionary sequence. Combining the HI observations with data from recent wide-field optical surveys, we evaluated the HI deficiencies of galaxies in a ~30' radius of the HCGs. We find that galaxies surrounding both phases exhibit similar distributions in their gas content. Similarly, galaxies making up the cores of Phase 2 HCGs are comparable to their neighbours in terms of HI deficiencies. However, Phase 3 groups are over an order of magnitude more deficient than their surroundings, supporting previous findings that late-phase HCG galaxies are more evolved than their large-scale environments.

==> tables/hidef_stats_core.tex <==
\begin{table}
\centering
\caption{Fractions of \hi-rich, normal and poor galaxies in the cores of the HCGs.}\label{tab:hidef_stats}
\begin{tabular}{l l c c c} 
\hline 
\hline 
Phase & HCG & \% rich & \% normal & \% poor \\ 
\hline
\multirow{3}{*}{2} & 16 & 60 & 0 & 40\\ 
 & 31 & 0 & 20 & 80\\ 
 & 91 & 25 & 50 & 25\\ 
\hline\multirow{3}{*}{3} & 30 & 0 & 0 & 100\\ 
 & 90 & 0 & 0 & 100\\ 
 & 97 & 0 & 20 & 80\\ 
\hline
\end{tabular}
\end{table}

==> tables/hidef_stats_out.tex <==
\begin{table}
\centering
\caption{Fractions of \hi-rich, normal and poor galaxies in the outskirts of the HCGs.}\label{tab:hidef_stats}
\begin{tabular}{l l c c c} 
\hline 
\hline 
Phase & HCG & \% rich & \% normal & \% poor \\ 
\hline
\multirow{3}{*}{2} & 16 & 11 & 11 & 77\\ 
 & 31 & 0 & 28 & 71\\ 
 & 91 & 53 & 7 & 38\\ 
\hline\multirow{3}{*}{3} & 30 & 42 & 14 & 42\\ 
 & 90 & 8 & 0 & 91\\ 
 & 97 & 20 & 6 & 73\\ 
\hline
\end{tabular}
\end{table}

==> tables/tab_mems_phase2.tex <==
\begin{table}
\begin{center}
\caption{\hi\ masses of individual HCG core members. The last two columns respectively list the \hi\ masses inside and outside the discs of the galaxies.}\label{tab:mems_phase2}
\begin{tabular}{l l c c} 
\hline 
\hline 
\multirow{2}{*}{HCG} & \multirow{2}{*}{member} & $\rm\log{M_{\textsc{Hi}, gal}}$ & $\rm\log{M_{\hi,ext}}$ \\ 
 & & $\rm (M_\odot)$ & $\rm (M_\odot)$ \\ 
\hline \rule{0pt}{10pt}
 \multirow{6}{*}{16} & 16A & 8.7 & --\\ 
 & 16B & 8.9 & -- \\ 
 & 16C & 9.6 & -- \\ 
 & 16D & 9.6 & -- \\ 
 & N0848 & 9.6 & -- \\ 
 & {\bf total} & {\bf 10.1} & {\bf 9.9}\\ 
\rule{0pt}{10pt}
 \multirow{6}{*}{31} & 31A & 8.5 & --\\ 
 & 31B & 8.9 & -- \\ 
 & 31C & 8.8 & -- \\ 
 & 31G & 8.6 & -- \\ 
 & 31Q & 8.5 & -- \\ 
 & {\bf total} & {\bf 9.4} & {\bf 10.2}\\ 
\rule{0pt}{10pt}
 \multirow{5}{*}{91} & 91A & 9.8 & --\\ 
 & 91B & 9.2 & -- \\ 
 & 91C & 9.6 & -- \\ 
 & WJ$^*$ & 8.2 & -- \\ 
 & {\bf total} & {\bf 10.1} & {\bf 9.8}\\ 
\hline
\rule{0pt}{10pt}
 \multirow{5}{*}{30} & 30A & ${<}7.4$ & --\\ 
 & 30B & ${}7.9$ & -- \\ 
 & 30C & ${<}7.5$ & -- \\ 
 & 30D & ${<}7.4$ & -- \\ 
 & {\bf total} & ${\bf {\leq}8.2}$ & {\bf --}\\ 
\rule{0pt}{10pt}
 \multirow{5}{*}{90} & 90A & ${}8.6$ & --\\ 
 & 90B & ${<}6.9$ & -- \\ 
 & 90C & ${<}6.9$ & -- \\ 
 & 90D & ${<}6.9$ & -- \\ 
 & {\bf total} & ${\bf {\leq}8.6}$ & {\bf 8.2}\\ 
\rule{0pt}{10pt}
 \multirow{6}{*}{97} & 97A & ${<}7.7$ & --\\ 
 & 97B & ${}8.9$ & -- \\ 
 & 97C & ${<}7.7$ & -- \\ 
 & 97D & ${<}7.7$ & -- \\ 
 & 97E & ${<}7.7$ & -- \\ 
 & {\bf total} & ${\bf {\leq}9.0}$ & {\bf --}\\ 
\hline
\end{tabular} \\ 
\rule{0pt}{10pt}
Note: $^*$WISEA J220854.95-274701.6 coincides spatially with the peak of an \hi\ cloud in the core of HCG 91, but lacks an optical readshift; we include it in this table but do not count it as a core member.
\end{center} 
\end{table}
